An Algebraic Framework for Runtime Verification

Runtime verification (RV) is a pragmatic and scalable, yet rigorous technique, to assess the correctness of complex systems, including cyber-physical systems (CPS). By measuring how robustly a CPS run satisfies a specification, RV allows in addition, to quantify the resiliency of a CPS to perturbations. In this paper we propose Algebraic Runtime Verification (ARV), a general, semantic framework for RV, which takes advantage of the monoidal structure of runs (w.r.t. concatenation) and the semiring structure of a specification automaton (w.r.t. choice and concatenation), to compute in an incremental and application specific fashion the resiliency measure. This allows us to expose the core aspects of RV, by developing an abstract monitoring algorithm, and to strengthen and unify the various qualitative and quantitative approaches to RV, by instantiating choice and concatenation with real-valued functions as dictated by the application. We demonstrate the power and effectiveness of our framework on two case studies from the automotive domain.

==> abstractRadu.tex <==
\begin{abstract}
Runtime verification (RV) is a pragmatic and scalable, yet rigorous
technique, to assess the correctness of complex systems, including
cyber-physical systems (CPS). In addition, by measuring how robustly a
CPS run satisfies a specification, RV allows to quantify the
resiliency of a CPS to perturbations. In this paper we propose a
general, semantic framework for RV, which takes advantage of the
monoidal structure of runs (with respect to concatenation) and the
semiring structure of a specification automaton (with repect to choice
and concatenation) to compute in an incremental and application
specific fashion the resiliency measure. This allows us to expose the
core aspects of RV, by developing an abstract monitoring algorithm, to
strengthen, and to unify the various qualitative and quantitative
approaches to RV, by instantiating choice and concatenation in this
algorithm, with real-valued functions as dictated by the
application. We demoonstrate the power and effectiveness of our
framework on two case studies from the automotive domain.
\end{abstract}


==> ezio.tex <==
%!TEX root = main.tex


\section{DNF minimization}
\label{sec:intervals}
\begin{definition}[Interval] An interval  is a connected subset in $\mathbb{R}$.  For simplicity, we refer to 
an interval with  the notation $[x]$ even when the interval is not closed.  We denote $\underline{x}$, $\bar{x}$  
as the lower and upper bound of an interval $[x]$, respectively:

$$ \underline{x} = lb ([x]) \triangleq \sup \{ a \in \mathbb{R}\; \cup \{ -\infty, +\infty \} \; |\; \forall x \in [x], a \leq x\}$$
$$ \bar{x} = ub ([x]) \triangleq \inf \{ b \in \mathbb{R}\; \cup \{ -\infty, +\infty \} \; |\; \forall x \in [x], x \leq b\}$$

\end{definition}

We write $[\underline{x}, \bar{x}]$,  $(\underline{x}, \bar{x}]$,  $[\underline{x}, \bar{x})$ and 
$(\underline{x}, \bar{x})$ to denote closed, right-open left-closed, 
left-open right-closed and open intervals, respectively.
We assume the empty set $\emptyset$ as a special kind of interval.  Then the set of intervals
is closed under the intersection defined as:
$$
[z] = [x] \cap [y] \triangleq  \{z \in \mathbb{R}\; | z \in [x] \wedge z \in [y]  \}
$$ 
The set of intervals is not closed under the union ($\cup$) and the complement ($[\;]^{c}$):
$$
[x]\; \cup \; [y] \triangleq  \{z \in \mathbb{R}\; | z \in [x] \vee z \in [y]  \},\;\;
[x]^{c} \triangleq  \{z \in \mathbb{R}\; | z \not\in [x]   \}
$$ 
\begin{example} Examples of intersection are $(2,5]\;\cap (3,6] = (3,5]$,  $(2,5]\;\cap (5,6] = \emptyset$.
The complement of a closed interval $[3,5]^{c} = (-\infty, 3) \cup (5,+\infty)$ is the union of two intervals: 
one left- and one right-unbounded. The complement of $(-\infty, +\infty)$ is $\varnothing$, while the 
complement of a left-unbounded right-closed interval $(-\infty, 3]$ is the left-open right-unbounded 
interval $(3, +\infty)$.
\end{example}

\begin{definition}[Interval vector] We define an interval vector $[\mathbf{x}] \subseteq \mathbb{R}^n$ 
as a Cartesian product of $n$ intervals:
$$[\mathbf{x}] = [x_1] \times [x_2] \times \cdots \times [x_n], \mbox{ with }  lb([x_i]) =  \underline{x_i}, ub([x_i]) = \bar{x_i}, \; \forall i = 1, \cdots, n$$
such that each \emph{i}th component $[x_i]$ is the projection of $[\mathbf{x}]$ onto the \emph{i}th axis.  
\end{definition}
Expressions such as $[\mathbf{x}] =   [3,4] \times \varnothing$ are indeed forbidden because $[3,4]$ is 
not a projection of $[\mathbf{x}]$ in the first axis.  We denote $\varnothing \times \cdots \times \varnothing$
as the empty set of $\mathbb{R}^n$. We define the intersection of two interval vectors $[\mathbf{x}] \subseteq \mathbb{R}^n$ and $[\mathbf{y}]  \subseteq \mathbb{R}^n$ as:

$$
[\mathbf{x}] \cap [\mathbf{y}] =     \left\{ \begin{array}{ll}
 [x_1]\; \cap\; [y_1]  \times [x_2] \cap [y_2] \times \cdots \times [x_n] \cap [y_n]  & \mbox{if }  \forall i, 1 \leq i \leq n,   [x_i] \cap [y_i] \neq \varnothing  \\ 
\varnothing  \times \varnothing \times \cdots \varnothing &   \mbox{otherwise}
\end{array}\right.$$
Algorithm~\ref{alg:complement} computes the complement of an interval vector 
$[\mathbf{x}]$ as illustrated in the figure on the right. The key idea is to enumerate and collect 
in a set all the possible interval vectors that can be generated by applying the cartesian 
product of the intervals in the complement of each component.  This algorithm requires 
$\mathcal{O} (3^n + 3n)$ operations, where $n$ is the number of components of the interval.


\begin{minipage}[h]{0.50\textwidth}
\begin{algorithm}[H]
\label{alg:complement}
\scriptsize

\caption{\textsf{compIntVec}$([\mathbf{x}])$}
\begin{algorithmic}[1]
\Require a vector of intervals \\ $[\mathbf{x}] =  [x_1] \times [x_2] \times \cdots \times  [x_n]$ 
\State
\State $F \gets \varnothing$
\State $c \gets 1$
\For{$i = 1~to~n$}
        \State $r_i \gets 0$
         \ForAll{$[y]  \in ([x_i] \cup [x_i]^c) $}
             \State $S_i(r_i) \gets [y] $;
             \State $r_i \gets r_i + 1$
         \EndFor
          \State $m_i = c$
          \State $c \gets c \cdot r_i$
\EndFor
\For{$j = 1~to~c$}
      
      \State $flag \gets 1$
      \For{$i = 1~to~n$}
           \State $[z_i] \gets S_i((j \div m_i) \mod r_i)$
           \If {($[z_i]  = \varnothing$)}
                 \State $flag \gets 0$
                 \State \textbf{break}
           \EndIf
      \EndFor
       \If {$(flag  = 1) \wedge ( [\mathbf{x}] \neq  [\mathbf{z}] )$}
           \State $F \gets F \cup ([z_1] \times [z_2] \times \cdots \times  [z_n])$
       \EndIf
\EndFor
\State \textbf{return} $F$



\end{algorithmic}
\end{algorithm}
\end{minipage}
\begin{minipage}[h]{0.50\textwidth}
\begin{center}


\begin{tikzpicture}



\draw[step=1cm,gray,very thin] (0,0) grid (6,6);
\filldraw [fill=black, draw=black, fill opacity=0.6] (2,2) rectangle (4,4);
    \node[draw,align=left,fill=white!20,scale=0.6] at (3,3) {$[2,4]\times[2,4]$};
    \node[draw,align=left,fill=white!20,scale=0.6] at (1,5) {$(-\infty,2)\times(4,+\infty)$};
    \node[draw,align=left,fill=white!20,scale=0.6] at (3,5) {$[2,4]\times(4,+\infty)$};
    \node[draw,align=left,fill=white!20,scale=0.6] at (5,5) {$(2,+\infty)\times(4,+\infty)$};
    
    
   \node[draw,align=left,fill=white!20,scale=0.6] at (1,1) {$(-\infty,2)\times(-\infty,2)$};
    \node[draw,align=left,fill=white!20,scale=0.6] at (3,1) {$[2,4]\times(-\infty,2)$};
    \node[draw,align=left,fill=white!20,scale=0.6] at (5,1) {$(2,+\infty)\times(-\infty,2)$};
    
   \node[draw,align=left,fill=white!20,scale=0.6] at (1,3) {$(-\infty,2)\times [2,4]$};
    \node[draw,align=left,fill=white!20,scale=0.6] at (5,3) {$(2,+\infty)\times [2,4]$};
    
\filldraw [fill=gray, draw=black, draw opacity=0.2,  fill opacity=0.2] (2,0) rectangle (4,2);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (2,4) rectangle (4,6);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (4,4) rectangle (6,6);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (4,2) rectangle (6,4);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (4,0) rectangle (6,2);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (0,0) rectangle (2,2);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (0,2) rectangle (2,4);
\filldraw [fill=gray, draw=black, draw opacity=0.2, fill opacity=0.2] (0,4) rectangle (2,6);
\draw[thick,->] (2,2) -- (-0.25,2);
\draw[thick,->] (2,4) -- (-0.25,4);
\draw[thick,->] (4,2) -- (6.25,2);
\draw[thick,->] (4,4) -- (6.25,4);
\draw[thick,->] (2,2) -- (2,-0.25);
\draw[thick,->] (4,2) -- (4,-0.25);
\draw[thick,->] (2,4) -- (2, 6.25);
\draw[thick,->] (4,4) -- (4, 6.25);

\node [below=1cm, align=flush center,text width=9.5cm, scale=0.8] at (3,8)
        {
            F = \textsf{compIntVec}$([2,4]\times[2,4]) $
        };
        
\node [below=1cm, align=flush center,text width=9.5cm, scale=0.6] at (3,0.5)
        {
            F = $\{ (-\infty,2)\times(4,+\infty), [2,4]\times(4,+\infty), (2,+\infty)\times(4,+\infty)$ \\ 
            
            $(-\infty,2)\times [2,4],(2,+\infty)\times [2,4] $ \\
            $ (-\infty,2)\times(-\infty,2), [2,4]\times(-\infty,2), (2,+\infty)\times(-\infty,2) \}$ \\ 
        };
\end{tikzpicture}
\end{center}
\end{minipage}

\begin{definition}[Predicate in Disjunctive Normal Form (DNF)]  A predicate in 
disjunctive normal form is generated by the following grammar:\\ \\
\fbox{\begin{minipage}{7em}
\footnotesize
$\psi  :=  \psi^{c}~|~\psi^{c} \vee \psi$
\end{minipage}}\hspace{4ex}
\fbox{\begin{minipage}{8em}
\footnotesize
$\psi^{c} :=  \psi^{l}~|~\psi^{l} \wedge \psi^{c} $
\end{minipage}}\hspace{4ex}
\fbox{\begin{minipage}{13em}
\footnotesize
$\psi^{l}  :=  \top~|~\bot~|~(x \preceq k)~|~\neg (x \preceq k)$
\end{minipage}}
%$$
%\begin{array}{lll}
%\psi & := & \psi^{c}~|~\psi^{c} \vee \psi \\
%\psi^{c} & := & \psi^{l}~|~\psi^{l} \wedge \psi^{c} \\
%\psi^{l} & := & \top~|~\bot~|~(x \preceq k)~|~\neg (x \preceq k)\\
%\end{array}
%$$

\noindent where $\preceq \in \{<, \leq\}$, $x \in \vars$ and $k \in \domain$. 
The predicate has indeed the following structure:

$$ \psi = \bigvee^{h}_{i=1} \psi^{c}_{i},\;\; \psi^{c}_{i} = \bigwedge^{m(i)}_{h=1}  \psi^{l}_{i,h}$$ where $h$ is the 
number of clauses, each clause $i$ is a conjunction of $m(i)$ literals and 
each literal can be either a basic proposition, its negation, true or false.  
\end{definition}

\begin{definition}[Predicate in Minimal DNF]  A predicate $\predicate$ is expressed in a 
minimal DNF if it satisfies the following properties:



$$ \left(  \bigwedge_{i=1}^{h} \bigwedge_{s=1,r = 1, s \neq r}^{m(i)} ( \psi^{l}_{i,s} \rightarrow \psi^{l}_{i,r})  = \bot \right)  \wedge  \left( \bigvee_{i=1,j=1, i \neq j}^{h}  ( \psi^{c}_{i} \wedge \psi^{c}_{j}) = \bot \right) $$

 \end{definition}
 
 \noindent The first expression in parenthesis on the left makes sure that in each conjunction there is not one 
 basic proposition that  implies another, while the second expression on right guarantees that all the conjunctions in the DNF
identify completely disjoint sets.
 
\begin{figure}
\begin{minipage}[h]{0.50\textwidth}
\begin{tikzpicture}

\usetikzlibrary{patterns}
\draw[step=0.25cm,gray,very thin] (0,0) grid (5.5,4);


        
\filldraw [fill=gray, draw=black, fill opacity=0.4] (2.5,0.5) rectangle (4,3.5);        

\node[draw,align=left,fill=white!20, scale=0.6, fill opacity=0.8] at (2.8,4.25) {a) Predicate $\predicate$ in DNF (Geometric Representation)};


\node[draw,align=left,fill=white!20, scale=0.55] at (2.75,3.75) {$\predicate_{1}^{c} = \neg (x < 2.5) \wedge (x \leq 4) \wedge \neg (y < 0.5) \wedge (y \leq 3.5)  $};

\filldraw [fill=orange, draw=black, fill opacity=0.4] (1.5,0.5) rectangle (4,2);
\draw [pattern=north west lines, pattern color=orange, draw=black] (1,0.5) rectangle  (1.5,2);


\node[draw,align=left,fill=white!20, scale=0.55] at (2.5,0.25) {$\predicate_{2}^{c} = \neg (x < 1) \wedge  \neg (x < 1.5) \wedge (x \leq 4) \wedge \neg (y < 0.5) \wedge (y \leq 2) $};
        
 \node[draw,align=left,fill=white!20, scale=0.7, fill opacity=0.8] at (1.25,2.75) {$ \predicate =  \predicate_{1}^{c}  \vee \predicate_{2}^{c} $};
 
 

 \node[draw,align=left, scale=0.55, fill=white!20, draw opacity=0.0] at (4.65,3.25) {$ x=3.25$ \\ $y=2.50$};
 
 \node[draw, color=red, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (3.7, 2.15) {$ - 0.5$};
 \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (2.9, 2.15) {$ 2.25$};
 \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (2.85, 2.65) {$ 0.75$};
  \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (3.7, 2.65) {$ 0.75$};
 \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (3.4, 3.20) {$ 1$};
        
     
 
\draw[thick,->] (0,0) -- (5.75,0);
\draw[thick,->] (0,0) -- (0,4.25);

\draw[very thin,-] (3.25,2.5)-- (4.1,3.25);
\draw[very thin,-] (4.1,3.25)-- (4.2,3.25);

\draw[thick, color=black,<->] (3.30,2.5) -- (4,2.5);
\draw[thick, color=black,<->] (3.21,2.5) -- (2.50,2.5);

\draw[thick, color=black,<->] (3.27,2.47) -- (3.27,0.5);
\draw[thick, color=red,<->] (3.38,2.47) -- (3.38,2);
\draw[thick, color=black,<->] (3.25,2.57) -- (3.25,3.5);

   \draw[red,fill=red] (3.25,2.5) circle (.4ex); 

\end{tikzpicture}
\end{minipage}
\begin{minipage}[h]{0.50\textwidth}
\begin{tikzpicture}
\draw[step=0.25cm,gray,very thin] (0,0) grid (5.5,4);

\filldraw [fill=gray, draw=black, fill opacity=0.4] (2.5,2) rectangle (4,3.5);        

\node[draw,align=left,fill=white!20, scale=0.6, fill opacity=0.8] at (2.8,4.25) {b) Predicate $\predicate'$ in Minimal DNF (Geometric Representation)};

\node[draw,align=left,fill=white!20, scale=0.55, fill opacity=0.8] at (2.5,3.75) {$\predicate_{1}^{c} = \neg (x < 2.5) \wedge (x \leq 4) \wedge \neg (y \leq 2) \wedge (y \leq 3.5) $};

\filldraw [fill=orange, draw=black, fill opacity=0.4] (1.5,0.5) rectangle (4,2);

\node[draw,align=left,fill=white!20, scale=0.55, fill opacity=0.8] at (2.5,0.25) {$\predicate_{2}^{c} = \neg (x < 1.5) \wedge (x \leq 4) \wedge \neg (y < 0.5) \wedge (y \leq 2) $};


        
 \node[draw,align=left,fill=white!20, scale=0.7, fill opacity=0.8] at (1.25,2.75) {$ \predicate' =  {\predicate'}_{1}^{c}  \vee {\predicate'}_{2}^{c} $};
 
 \node[draw,align=left, scale=0.55, fill=white!20, draw opacity=0.0] at (4.65,3.25) {$ x=3.25$ \\ $y=2.50$};
 
 \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (3.5, 2.15) {$0.5$};
 \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (2.85, 2.65) {$ 0.75$};
  \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (3.7, 2.65) {$ 0.75$};
 \node[draw, color=black, fill=white!20, align=right, scale=0.55, draw opacity=0.0] at (3.4, 3.20) {$ 1$};
        
     
 
\draw[thick,->] (0,0) -- (5.75,0);
\draw[thick,->] (0,0) -- (0,4.25);

\draw[very thin,-] (3.25,2.5)-- (4.1,3.25);
\draw[very thin,-] (4.1,3.25)-- (4.2,3.25);

\draw[thick, color=black,<->] (3.30,2.5) -- (4,2.5);
\draw[thick, color=black,<->] (3.21,2.5) -- (2.50,2.5);

\draw[thick, color=black,<->] (3.25,2.47) -- (3.25,2);
\draw[thick, color=black,<->] (3.25,2.57) -- (3.25,3.5);

   \draw[red,fill=red] (3.25,2.5) circle (.4ex); 
\end{tikzpicture}
\end{minipage}
\caption{Geometric representation of the predicate $\predicate$ in DNF (a) and one possible 
equivalent $\predicate'$ in minimal DNF.}
\label{fig:minimal_dnf}
\end{figure}

\noindent Fig.~\ref{fig:minimal_dnf} shows an example of a predicate $\predicate$ in DNF that is not minimal for two reasons:
(1) $\neg (x < 1.5) \rightarrow \neg (x < 1) $ and (2) $\predicate_{1}^{c} \wedge \predicate_{2}^{c} \neq \bot$. On the other hand, 
$\predicate'$ is a minimal DNF and $\predicate' \equiv \predicate$.  Given an assignment ($x=3.25, y=2.50$) if we interpret the predicate
$\predicate$ and  $\predicate'$ using the idempotent MinMax semiring (instead of the Boolean one) we would 
obtain two different values: $0.75$ for $\predicate$ and $0.5$ for $\predicate'$. This shows that the 
minimal DNF can enable more precision in the quantitative assessment of the formula also with idempotent semirings. However, 
we can show that there could be several minimal DNF formulas equivalent to the original $\predicate$ and in 
some cases the precision in the quantitative assessment using idempotent semirings is 
the same as the original one.  An example is the following predicate $\predicate''$ that is 
a minimal DNF logically equivalent to $\predicate$:

$$\predicate'' = (\neg (x < 1.5) \wedge (x < 2.5) \wedge \neg (y < 0.5) \wedge (y \leq 2)) \vee $$
$$ (\neg (x < 2.5) \wedge (x \leq 4) \wedge \neg (y \leq 0.5) \wedge (y \leq 3.5)) $$

  \begin{proposition} Given a predicate $\predicate$ in DNF, there is an algorithm (that we call \textsf{minimalDNF}) to transform $\predicate$ in 
 another equivalent predicate $\predicate' \equiv \predicate$ that is in minimal DNF.  The time complexity of this algorithm 
 is $\mathcal{O}(\frac{1-(3^n + 3n + m_{max})^{h}}{1-(3^n + 3n + m_{max})})$ where $n$ is the number of variables, $h$ is the number of conjunctions
 and $m_{max}$ is the maximum number of terms that can appear in one the $h$ conjunctions.
 

 \end{proposition}
 
\begin{proof}
 $$\sum_{k=0}^{h-1} a^k = \frac{1-a^{h}}{1-a}$$
 $$ a = (3^n + 3n) $$
 $$\sum_{k=1}^{h-1} (3^n + 3n)^k = \frac{1-(3^n + 3n)^{h}}{1-(3^n + 3n)}$$
\end{proof}

\begin{minipage}[t]{0.50\textwidth}
\begin{algorithm}[H]
\scriptsize

\caption{\textsf{DNF2IntVecSet}$(S, \predicate)$}
\begin{algorithmic}[1]
\State $S' \gets \varnothing$
\State $[\mathbf{z}] \gets (-\infty, +\infty) \times \cdots \times (-\infty, +\infty)$
\If {($\predicate = \predicate_c \vee \predicate'$) or ($\predicate = \predicate_c$)}
    \State $[\mathbf{x}] \gets$  \textsf{conj2IntVec}$([\mathbf{z}],\predicate_c)$
    \State $S' \gets S' \cup [\mathbf{x}] $
    \If {($[\mathbf{x}] = [\mathbf{z}]$)}
           \State \textbf{return} $S'$
    \EndIf 
     \If {($[\mathbf{x}] \neq \varnothing \times \cdots \times \varnothing$)}
          \State $C \gets$ \textsf{compIntVec}$([\mathbf{x}]))$
          \ForAll{$[\mathbf{y}]  \in S$}
            \State $S' \gets S' \cup ([\mathbf{y}] \cap C$) 
         \EndFor
         \State $S \gets S' $         
    \EndIf 
\EndIf 
\If {($\predicate = \predicate_c \vee \predicate'$)}
 \State \textbf{return} \textsf{dnf2IntVecSet}$(S, \predicate')$
\EndIf 
    \State \textbf{return} $S$

\end{algorithmic}
\end{algorithm}

\vspace{-10ex}
\begin{algorithm}[H]
\scriptsize

  \caption{\textsf{conj2IntVec}$([\mathbf{x}],\predicate_c)$}
\begin{algorithmic}[1]

\If {($\predicate_c = \top $)}
      \State \textbf{return} $[x_1] \times [x_2] \times \cdots \times [x_n]$
\ElsIf  {($\predicate_c = \bot $)}     
      \State \textbf{return} $\varnothing \times \varnothing \times \cdots \varnothing$
\ElsIf  {($\predicate_c = x_i \preceq k$) $\vee$ ($\predicate_c = \neg (x_i \preceq k)$)}

           \State $[x_i] \gets [x_i]\; \cap $ \textsf{lit2Int}$(\predicate_{c})$ 
       \If {($[x_i] = \varnothing$)}
        \State \textbf{return}   $\varnothing \times \varnothing \times \cdots \varnothing$
    \EndIf 

\ElsIf {($\predicate_c =\predicate_{l} \wedge \predicate_{c} $)}
         \State $[\mathbf{y}] \gets \textsf{conj2IntVec}([\mathbf{x}],\predicate_l)$
          \State $[\mathbf{z}] \gets \textsf{conj2IntVec}([\mathbf{x}],\predicate_c)$
          \For{$i = 1~to~n$}
          \State $[x_i] =  [y_i] \cap [z_i] $
          \If {($[x_i] = \varnothing$)}
          \State \textbf{return}  $\varnothing \times \varnothing \times \cdots \varnothing$
           \EndIf   
          \EndFor
\EndIf
\State \textbf{return} $[x_1] \times [x_2] \times \cdots \times [x_n]$


\end{algorithmic}
\label{alg:conj2IntVec}


\end{algorithm}
\end{minipage}
%
~
\begin{minipage}[t]{0.55\textwidth}
\begin{algorithm}[H]
\scriptsize

\caption{\textsf{lit2int}$(\predicate_{l})$}
\begin{algorithmic}[1]
\State
\If  {($\predicate_l = x \preceq k$)}
           \State \textbf{return} $ (\preceq = '<')\; ?\; (-\infty, k) : (-\infty, k]$
\ElsIf  {($\predicate_l = \neg(x \preceq k)$)}
          \State \textbf{return}  $ (\preceq = '<')\; ?\;  [k, +\infty) : (k, +\infty)$
\EndIf 
\end{algorithmic}
\label{alg:lit2int}
\end{algorithm}
\vspace{-10ex}

\begin{algorithm}[H]
\caption{\textsf{intVecSet2DNF}$(S)$}
\begin{algorithmic}[1]
\scriptsize
\State $\predicate \gets \bot$ 

 \ForAll{$[\mathbf{x}]  \in S$}
 
 \State $\predicate_c = \top$
 \For{$i = 1~to~n$}
 \State $\predicate' \gets null$
  \If  {($[x_i] = \varnothing $)}
   \State $\predicate_c \gets null$
   \State \textbf{break} 
 \ElsIf  {($[x_i] = [\underline{x}_i, \bar{x}_i] $)}
 \State $\psi' \gets (x_i \leq \bar{x}_i) \wedge \neg (x_i < \underline{x}_i) $
 \ElsIf  {($[x_i] = (\underline{x}_i, \bar{x}_i) \wedge \underline{x}_i \neq  \bar{x}_i$)}
   \If  {($\underline{x}_i = - \infty \wedge  \bar{x}_i \neq + \infty $)}
    \State $\psi' \gets (x_i < \bar{x}_i) $
   \ElsIf  {($\underline{x}_i \neq - \infty \wedge  \bar{x}_i = + \infty $)}
        \State $\psi' \gets \neg (x_i \leq \underline{x}_i) $
     \ElsIf  {($\underline{x}_i \neq - \infty \wedge  \bar{x}_i \neq + \infty $)}
            \State $\psi' \gets (x_i < \bar{x}_i) \wedge \neg (x_i \leq \underline{x}_i) $
   \EndIf
 \ElsIf  {($[x_i] = [\underline{x}_i, \bar{x}_i)$)}
        \State $\psi' \gets \neg (x_i < \underline{x}_i) $
        \If  {($ \bar{x}_i \neq + \infty $)}
         \State $\psi' \gets \psi' \wedge   (x_i < \bar{x}_i) $
        \EndIf
 \ElsIf  {($[x_i] = (\underline{x}_i, \bar{x}_i]$)}
         \State $\psi' \gets (x_i \leq \bar{x}_i) $
          \If  {($ \underline{x}_i \neq - \infty $)}
         \State $\psi' \gets \psi' \wedge \neg (x_i \leq \underline{x}_i) $
        \EndIf
 \EndIf
 \If  {($ \psi' \neq null $)}
              \State $ \predicate_c \gets ( \predicate_c  = \top ) \; ?\; \psi' : \predicate_c \wedge \psi'  $
  \EndIf
 \EndFor
 
 \State  $\predicate  \gets ( \predicate  = \bot  ) \; ?\; \predicate_c :  \predicate \vee \predicate_c $
  \EndFor
   \State \textbf{return} $\predicate$
 \end{algorithmic}

\end{algorithm}
\vspace{-10ex}
\begin{algorithm}[H]
\caption{\textsf{minimalDNF}$(\predicate)$}
\begin{algorithmic}[1]
\scriptsize
\State $S \gets $ \textsf{DNF2IntVecSet}$(\varnothing, \predicate)$
\State \textbf{return} \textsf{intVecSet2DNF}$(S)$
 \end{algorithmic}

\end{algorithm}
\end{minipage}







 
 
 

==> proof.tex <==
\newpage

\section{Appendix: Correctness Conditions}
\label{sec:correctness}
This appendix will list the necessary conditions for algorithm correctness.


\begin{enumerate}
\item $\oone=0$.

This is necessary in order to ensure Algorithm~\ref{alg:val} returns zero distance when valuation $\val$ is in the set specified by $\psi$. This also ensures that such $\val$ does not
add to the path cost when we apply operation $\otimes$. 

%\item $\boxone$ is annihilator for $\boxplus$.

%If we have a satisfying trace it should have zero-cost which annihilates the costs incurred by other traces. 
%This implies that $\boxone$ must be annihilator for operation $\boxplus$.

\item $\oplus$ is idempotent. 

This is required to prove the Base Case 1, in proof for Theorem 1. The relation which we need to prove using idempotence:
$\mathlarger{\oplus}_{v' \models x_i \preceq k}  ~d(v_{(x_i)}, v'_{(x_i)}) \Leftrightarrow d(\val_{(x_i)}, k)$. It is also important to note that idempotent $\oplus$ requirement comes naturally from the robustness definition which is based on word-set distance function: the distance is equal to the \textit{minimal} word-to-word distance. 

Another reason why this is the necessary requirement is the following: in case we have non-idempotent $\oplus$ then the cost we get depend on the structure of the automaton. In example, if we have two semantically equivallent automata they would calculate different cost. What would happen in case of non-deterministic WSA?

\item $\oone$ is annihilator for $\oplus$.

%Let us take a $\predicate = x > k_1 \wedge x < k_2$ and $ k_1 < k_2$ and we take a valuation over $x$ , $\val_(x) < k_1$.
% In this case $d(\val, \predicate)$ is not influenced by $d(\val, x<k_2)$ which needs to be resolved to identity element $\oone$. 
Distance of a word from a set is calculated according to Definition~\ref{def:pred-val}. Let's assume now that we have a word which is in the set $\predicate$. Then, the distance of this word from the set must annihilate the distances of all the other words from the same set which participate in $\oplus$-sum in Definition~\ref{def:pred-val}. This is a necessary condition for the Lemma~\ref{lemma1} to hold. 

\item $\predicate$ must be minimal DNF.

Non-minimal $\predicate$ implies the conjunctions in $\predicate$ are not minimal. Then, we get incorrect result when we use non-idempotent $\otimes$ (i.e. Tropical Semiring used to calculate Hamming distance). On the other hand, for idempotent $\otimes$ the conjunctions need not to be minimal.

\end{enumerate}

Some further discussion of the results:
\begin{enumerate}
\item In case of non-idempotent $\oplus$, we have to define minimization procedure over the disjuncts of the $\predicate$ in order to obtain the correct robustness degree. 
\item 
In case $\oplus$ is not idempotent, the algorithm would not calculate the robustness degree anymore. Instead of calculating distance-based the robustness degree, which is by defintion founded on minimum (idempotent operation) word-set distance, it would calculate an additive property (i.e. probability).
\item We must precisely define that the val-pred distance returns $\oone = 0$ when valuation is in the set.
\end{enumerate}




\section{Appendix: Theorem Proofs}
\label{sec:proofs}

%\begin{nnprop}
%The weighted edit distance is a distance.
%\end{nnprop}
%
%\begin{proof}
%
%The proof is similar to the proof that edit distance is a distance, and is given for completeness reason.
%\begin{enumerate}
%\item $d_{W}(s,s) = 0:$ in order to transform $s$ to itself, no insertions or deletions are needed, and all substitutions have cost $0$.
%\item $d_{W}(s_{1},s_{2}) = d_{W}(s_{2},s_{1}):$ insertions and deletions are inverses of each other, while substitution is symmetric. 
%\item $d_{W}(s_{1},s_{2}) \geq 0:$ by definition, all costs are greater or equal to $0$.
%\item $d_{W}(s_{1}, s_{2}) \leq d_{W}(s_{1}, s) + d_{W}(s,s_{2}) :$ by definition, $d_{W}(s_{1},s_{2})$ is the minimum summation of 
%insertion, deletion and substitution costs needed to transform $s_{1}$ to $s_{2}$. Transforming $s_{1}$ to $s$, and then $s$ to $s_{2}$ 
%is one way of transforming $s_{1}$ to $s_{2}$, and hence cannot be cheaper than $d_{W}(s_{1}, s_{2})$.
%\end{enumerate}
%\end{proof} \qed

 

For the next theorem, we first prove an auxiliary lemma.

\begin{nnlem} 
\label{lemma1}
For distance function $d$, valuations $\val, \val'$ and operators $\otimes$ and $\oplus$ the following relation holds:


\begin{tabular}{l}
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}\mathlarger{\otimes}_{x \in \vars}~d(\val,\val') = 
\mathlarger{\oplus}_{\val' \models \psi_1} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')~\otimes~
\mathlarger{\oplus}_{\val' \models \psi_2} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$\\
\end{tabular}


\noindent where $\psi_1 \wedge \psi_2$ is a P-term from minimal DNF formula $\psi$.
\end{nnlem}

\begin{proof}
Since $\psi_1 \wedge \psi_2$ is a part of a minimal formula, it is satisfiable and it takes the form 
$ ( x_{i} > k_{1} \wedge x_{j} < k_{2} )$, where $k_1 < k_2$. We shall transform left hand side and right hand side of Lemma~\ref{lemma1} separately, in order to prove equivalence. We reason by cases. There are two distinct cases: (1) $x_{i} = x_{j}$ and (2)  $x_{i} \neq x_{j}$. 
 
\noindent \textbf{Case 1: $x_{i} = x_{j}$}. 
Since we have clauses specified over a single variable $x_{i}$, we can substitute 
$\mathlarger{\otimes}_{x \in \vars}~d(\val,\val') = d(\val_{(x)},\val'_{(x)}) = d(\val,\val').$

\noindent (a) Let us take an arbitrary $\val < k_1$. For the left hand side(LHS) of Lemma~\ref{lemma1}, directly from Definition~\ref{def:distance}, equality (4), follows that
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}~d(\val,\val')$ = $d(v, k_1)$. For the right hand side(RHS): 

 
 
\vspace{2pt}
\noindent
\begin{tabular}{l c l c l}
$\mathlarger{\oplus}_{\val' \models \psi_1}d(\val,\val')$  &  $~\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} d(\val,\val')$  &   ~$\Leftrightarrow$~	 & Def.~\ref{def:distance}\\

$  d(v, k_1)                                                               $  &  $~\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} d(\val,\val')$  &   ~$\Leftrightarrow$~	 & $\oplus$ is associative \\

$  d(v, k_1)                                                               $  &  $~\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2 s.t. \val' \neq \val''} d(\val,\val')  \oplus d(\val,\val'') $ &   ~$\Leftrightarrow$~	 & $\val < k_1 \wedge \psi_2=\val<k_2 \wedge k_1<k_2 \wedge v''=\val$  \\

$  d(v, k_1)                                                               $  &  $~\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2 s.t. \val' \neq \val} d(\val,\val')  \oplus d(\val,\val) $  &   ~$\Leftrightarrow$~	 &  Def.~\ref{def:distance} \\
$  d(v, k_1)                                                               $ &  $~\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2 s.t. \val' \neq \val} d(\val,\val')  \oplus \oone $  &   ~$\Leftrightarrow$~  & $\oone$ is   annihilator for $\oplus$	 \\ 
$  d(v, k_1)                                                               $ & $~\otimes$~ & $ \oone $ & ~$\Leftrightarrow$~ & identity element for $\otimes$ 	 \\ 
$  d(v, k_1)                                                               $ \\
\end{tabular}
\vspace{2pt}



\noindent (b) Let us take an arbitrary $\val$ s.t. $k_1 \leq \val \leq  k_2$. Since $\val \models \psi_1$ and $\val \models \psi_2$, directly from Definition~\ref{def:distance}, equality (4), follows that $\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}~d(\val,\val')$ = $\oone$. For the right hand side: 

 
 
\vspace{2pt}
\noindent
\begin{tabular}{lclcl}
$\mathlarger{\oplus}_{\val' \models \psi_1}d(\val,\val')$&$~\otimes~$&$\mathlarger{\oplus}_{\val' \models \psi_2} d(\val,\val') $ & ~$\Leftrightarrow$~	 & $\oplus$ is associative \\

$\mathlarger{\oplus}_{\val' \models \psi_1 s.t. \val' \neq \val''} d(\val,\val')  \oplus d(\val,\val'') $   &$~\otimes~$&  $\mathlarger{\oplus}_{\val' \models \psi_2 s.t. \val' \neq \val''} d(\val,\val')  \oplus d(\val,\val'') $ & ~$\Leftrightarrow$~	 &  $k_1 \leq \val \leq  k_2; v'' = \val$\\

$\mathlarger{\oplus}_{\val' \models \psi_1 s.t. \val' \neq \val} d(\val,\val')  \oplus d(\val,\val) $   &$~\otimes~$&  $\mathlarger{\oplus}_{\val' \models \psi_2 s.t. \val' \neq \val} d(\val,\val')  \oplus d(\val,\val) $ & ~$\Leftrightarrow$~	 &  Def.~\ref{def:distance}\\

$\mathlarger{\oplus}_{\val' \models \psi_1 s.t. \val' \neq \val''} d(\val,\val')  \oplus \oone $   &$~\otimes~$&  $\mathlarger{\oplus}_{\val' \models \psi_2 s.t. \val' \neq \val''} d(\val,\val')  \oplus \oone $ & ~$\Leftrightarrow$~	 &   $\oone$ is   annihilator for $\oplus$\\



$  \oone                                                              $&$\otimes$&$ \oone $ & ~$\Leftrightarrow$~ &  identity element for $\otimes$ 	 \\ 
$  \oone                                                               $ \\
\end{tabular}
 \vspace{2pt}

\noindent (c) Let us take an arbitrary $\val > k_2$. Then, directly from Definition~\ref{def:distance}, equality (4), follows that
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}~d(\val,\val')$ = $d(v, k_2)$. For the right hand side: 


\vspace{2pt}
\noindent
\begin{tabular}{l c l c l}
$\mathlarger{\oplus}_{\val' \models \psi_1}d(\val,\val')$  &  $~\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} d(\val,\val')$  &   ~$\Leftrightarrow$~	 & Def.~\ref{def:distance}\\

$ \mathlarger{\oplus}_{\val' \models \psi_1}d(\val,\val') $  &  $~\otimes$~ &  $d(v, k_2)$  													          &   ~$\Leftrightarrow$~	 & $\oplus$ is associative \\

$\mathlarger{\oplus}_{\val' \models \psi_1 s.t. \val' \neq \val''} d(\val,\val')  \oplus d(\val,\val'') $  &  $~\otimes$~ &  $d(v, k_2)$          &   ~$\Leftrightarrow$~	 & $\val > k_2 \wedge \psi_1=\val>k_1 \wedge k_1<k_2 \wedge v''=\val$  \\
$\mathlarger{\oplus}_{\val' \models \psi_1 s.t. \val' \neq \val''} d(\val,\val')  \oplus d(\val,\val) $   &  $~\otimes$~ &  $d(v, k_2)$          &   ~$\Leftrightarrow$~	 &  Def.~\ref{def:distance}  \\
$\mathlarger{\oplus}_{\val' \models \psi_1 s.t. \val' \neq \val''} d(\val,\val')  \oplus \oone $   &  $~\otimes$~ &  $d(v, k_2)$          &   ~$\Leftrightarrow$~	 &  $\oone$ is   annihilator for $\oplus$  \\
$\oone $   &  $~\otimes$~ &  $d(v, k_2)$          &   ~$\Leftrightarrow$~	 &  identity element for $\otimes$  \\
$d(v, k_2)$   &   &            &    	 &   

\end{tabular}
\vspace{2pt}

For Case 1, Lemma~\ref{lemma1} holds.



%s\newpage
\noindent \textbf{Case 2: $x_{i} \neq x_{j}$}. 

%A
\noindent (a) $\val_{(x_i)} \not\models \psi_1 \wedge \val_{(x_j)} \not\models \psi_2$

LHS: 

\begin{tabular}{r l l }
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}\mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &     ~$\Leftrightarrow$~     &    Def.~\ref{def:pred}\\
$\mathlarger{\oplus}_{\val' \models  ( x_i \preceq k_1 \wedge x_j \preceq k_2  ) }\mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &     ~$\Leftrightarrow$~    \\
$\mathlarger{\oplus}_{\val' \models  ( x_i \preceq k_1 \wedge x_j \preceq k_2  ) }(   d(\val_{(x_i)},\val'_{(x_i)}) \otimes d(\val_{(x_j)},\val'_{(x_j)}) ) $ &     ~$\Leftrightarrow$~    & Def.~\ref{def:distance}.(4)\\

%$\mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ s.t. $\val' = \{ x_i = k_1, x_j = k_2  \} $ &     ~$\Leftrightarrow$~    \\
$d(\val_{(x_i)},k_i) \otimes d(\val_{(x_j)},k_j)$									    

\end{tabular}

RHS: 

\begin{tabular}{r l l l r}
$\mathlarger{\oplus}_{\val' \models \psi_1} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ & ~$\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &
~$\Leftrightarrow$~       \\

$\mathlarger{\oplus}_{\val' \models x_i \preceq k_1} \mathlarger{\otimes}_{x_i}~d(\val,\val')$ &~$\otimes$~ & $ \mathlarger{\oplus}_{\val' \models x_j \preceq k_2} \mathlarger{\otimes}_{x_j}~d(\val,\val')$ &    ~$\Leftrightarrow$~       \\
$\mathlarger{\oplus}_{\val' \models x_i \preceq k_1} ~d(\val_{(x_i)},\val'_{(x_i)})$ &~$\otimes$~ & $ \mathlarger{\oplus}_{\val' \models x_j \preceq k_2} ~d(\val_{(x_j)},\val'_{(x_j)})$ &    ~$\Leftrightarrow$~       &       Def.~\ref{def:distance}.(4) \\
$d(\val_{(x_i)},k_i) $ &~$\otimes$~ & $d(\val_{(x_j)},k_j)$									    


\end{tabular}

%B
\noindent (b) $\val_{(x_i)} \not\models \psi_1 \wedge \val_{(x_j)} \models \psi_2$

LHS: 

\begin{tabular}{r l l l r}
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}\mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &     ~$\Leftrightarrow$~     &    Case 2.a\\
$d(\val_{(x_i)},k_i) \otimes d(\val_{(x_j)},k_j)$ & ~$\Leftrightarrow$~     &   $ \val_{(x_j)} \models \psi_2 \wedge$ Def.~\ref{def:distance}\\
$d(\val_{(x_i)},k_i) \otimes \oone $  & ~$\Leftrightarrow$~     &   $\oone$ is identity element for $\otimes$ \\
$d(\val_{(x_i)},k_i)                      $       \\

\end{tabular}

RHS: 

\begin{tabular}{rllll}
$\mathlarger{\oplus}_{\val' \models \psi_1} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ & ~$\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &
~$\Leftrightarrow$~ & Case 2.a     \\

$d(\val_{(x_i)},k_i) $ &~$\otimes$~ & $d(\val_{(x_j)},k_j)$  &  ~$\Leftrightarrow$~ & $\val_{(x_j)} \models \psi_2$; Def.~\ref{def:distance}     \\
$d(\val_{(x_i)},k_i) $ &~$\otimes$~ & $ \oone $  & ~$\Leftrightarrow$~ & $\oone$ is identity element \\
$d(\val_{(x_i)},k_i)                      $       \\


\end{tabular}

%C
\noindent (c) $\val_{(x_i)} \models \psi_1 \wedge \val_{(x_j)} \not\models \psi_2$

LHS: 

\begin{tabular}{rllll}
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}\mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &     ~$\Leftrightarrow$~ &    Case 2.a\\
$d(\val_{(x_i)},k_i) \otimes d(\val_{(x_j)},k_j)$ & ~$\Leftrightarrow$~     &   $ \val_{(x_i)} \models \psi_1 \wedge$ Def.~\ref{def:distance}\\
$\oone \otimes d(\val_{(x_j)},k_j) $  & ~$\Leftrightarrow$~     &   $\oone$ is identity element for $\otimes$ \\
$d(\val_{(x_j)},k_j)                    $       \\

\end{tabular}

RHS: 

\begin{tabular}{rllll}
$\mathlarger{\oplus}_{\val' \models \psi_1} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ & ~$\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &
~$\Leftrightarrow$~ & Case 2.a     \\

$d(\val_{(x_i)},k_i) $ &~$\otimes$~ & $d(\val_{(x_j)},k_j)$  &  ~$\Leftrightarrow$~ & $\val_{(x_i)} \models \psi_1$; Def.~\ref{def:distance}     \\
$\oone $ &~$\otimes$~ & $ d(\val_{(x_j)},k_j) $  & ~$\Leftrightarrow$~     &   $\oone$ is identity element for $\otimes$ \\
$d(\val_{(x_j)},k_j)                    $       \\
\end{tabular}

%D
\noindent (d) $\val_{(x_i)} \models \psi_1 \wedge \val_{(x_j)} \models \psi_2$

LHS: 

\begin{tabular}{rllll}
$\mathlarger{\oplus}_{\val' \models \psi_1 \wedge \psi_2}\mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &     ~$\Leftrightarrow$~     &    Case 2.a\\
$d(\val_{(x_i)},k_i) \otimes d(\val_{(x_j)},k_j)$ & ~$\Leftrightarrow$~     &   $ \val_{(x_i)} \models \psi_1 \wedge  \val_{(x_j)} \models \psi_2 \wedge$ Def.~\ref{def:distance}\\
$\oone \otimes \oone $  & ~$\Leftrightarrow$~     &   $\oone$ is identity element for $\otimes$ \\
$\oone                    $       \\

\end{tabular}

RHS: 

\begin{tabular}{rllll}
$\mathlarger{\oplus}_{\val' \models \psi_1} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ & ~$\otimes$~ & $\mathlarger{\oplus}_{\val' \models \psi_2} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$ &
~$\Leftrightarrow$~ & Case 2.a     \\

$d(\val_{(x_i)},k_i) $ &~$\otimes$~ & $d(\val_{(x_j)},k_j)$  &  ~$\Leftrightarrow$~ & $ \val_{(x_i)} \models \psi_1 \wedge  \val_{(x_j)} \models \psi_2 \wedge$ Def.~\ref{def:distance}     \\
$\oone $ &~$\otimes$~ & $ \oone $  & ~$\Leftrightarrow$~     &   $\oone$ is identity element for $\otimes$ \\
$\oone                    $       \\
\end{tabular}

For Case 2, Lemma~\ref{lemma1} holds.

\end{proof} \qed

   


%%%%-----------------------------------------------------------------------

\begin{nnlem} 
\label{lemma2}
For operator $\oplus$ from an additively-idempotent semiring $\algebra$ and a value $\val$ from the semiring domain, the following relation holds:


%\begin{tabular}{l}
%$\mathlarger{\oplus}_{\val' \models \psi_1 \vee \psi_2}\mathlarger{\otimes}_{x \in \vars}~d(\val,\val') = 
%\mathlarger{\oplus}_{\val' \models \psi_1} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')~\oplus~
%\mathlarger{\oplus}_{\val' \models \psi_2} \mathlarger{\otimes}_{x \in \vars}~d(\val,\val')$\\
%\end{tabular}

\begin{tabular}{l}
$\mathlarger{\oplus}_{\val \models \psi_1 \vee \psi_2}~\val = 
\mathlarger{\oplus}_{\val \models \psi_1}~\val  ~\oplus~
\mathlarger{\oplus}_{\val \models \psi_2}~\val $\\
\end{tabular}

\noindent where $\psi_1 \vee \psi_2$ is a minimal DNF.
\end{nnlem}


\begin{proof}
Based on semantics of $\models$ relation, we reduce logical operations over constraints to operations over (finite or infinite) sets. 
We use $F_1$ and $F_2$ to designate the sets of words specified by logical constraints  $\psi_1 $  and $\psi_2$, respectfully.

\begin{tabular}{cllll}
$\mathlarger{\oplus}_{\val \models \psi_1 \vee \psi_2}~\val $ & &    &       ~$\Leftrightarrow$~     & semantics of $\models$  \\
$\mathlarger{\oplus}_{\val \in F_1 \cup F_2}~\val $                & &    &    ~$\Leftrightarrow$~     & semantics of $\cup, \setminus , \cap$     \\
$\oplus_{\val \in F_1 \setminus F_2}~\val$  $~\mathlarger{\oplus}~$  $ \oplus_{\val \in F_1 \cap F_2}~\val ~\mathlarger{\oplus}~ \oplus_{\val \in F_2 \setminus F_1}~\val  $
\end{tabular}

We distinguish two cases depending on whether $F_1$ and $F_2$ intersect or not.

\noindent \textbf{Case 1: $ F_1 \cap F_2 = \lbrace \emptyset \rbrace$}. 

\begin{tabular}{rllllll}
$\oplus_{\val \in F_1 \setminus F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_1 \cap F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_2 \setminus F_1}~\val$ &  ~$\Leftrightarrow$~   & semantics of $\cup, \setminus , \cap $ \\ 
$\oplus_{\val \in F_1 \setminus F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_2 \setminus F_1}~\val$ & & & ~$\Leftrightarrow$~     &  $ F_1 \cap F_2 = \lbrace \emptyset \rbrace$ \\ 
$\oplus_{\val \models \psi_1}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \models \psi_2}~\val$
\end{tabular}


\noindent \textbf{Case 2: $ F_1 \cap F_2 \neq \lbrace \emptyset \rbrace $}. 

\begin{tabular}{rlllllllll}
$\oplus_{\val \in F_1 \setminus F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_1 \cap F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_2 \setminus F_1}~\val$ & & & ~$\Leftrightarrow$~   & idempotence of $\oplus$\\ 
$\oplus_{\val \in F_1 \setminus F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_1 \cap F_2}~\val$ & $~\mathlarger{\oplus}~$ & $\oplus_{\val \in F_1 \cap F_2}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_2 \setminus F_1}~\val$ &  ~$\Leftrightarrow$~   & semantics of $\cup, \setminus , \cap $ \\ 
$\oplus_{\val \in F_1}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \in F_2}~\val$ & & & & & ~$\Leftrightarrow$~     &  $ F_1 \cap F_2 \neq \lbrace \emptyset \rbrace$ \\ 
$\oplus_{\val \models \psi_1}~\val$ & $~\mathlarger{\oplus}~$  & $\oplus_{\val \models \psi_2}~\val$
\end{tabular}

\end{proof} \qed


%%%%-----------------------------------------------------------------------





\begin{customthm}{\ref{thm:valpred}}
$\textsf{vpd}(\val, \predicate)$ = $d(\val, \predicate)$
\end{customthm}
\begin{proof} We shall prove this theorem using structural induction on the $ \predicate$ syntax specified in Definition~\ref{def:pred}.

\noindent \textit{Base Case 1}: Theorem~\ref{thm:valpred} holds for arbitrary $\predicate = x_i \preceq k$. 

\noindent \textit{Proof}. Let's expand the LHS of Theorem~\ref{thm:valpred}:

\begin{tabular}{c l lll }
$d(\val, \predicate)$ & ~$\Leftrightarrow$~ & Def~\ref{def:pred-val} \\
$\mathlarger{\oplus}_{v' \models \psi}  \mathlarger{\otimes}_{x \in \vars} ~d(v_{(x)}, v'_{(x)})$ & ~$\Leftrightarrow$~ &   $\predicate = x_i \preceq k$ \\
$\mathlarger{\oplus}_{v' \models x_i \preceq k}  \mathlarger{\otimes}_{x \in \vars} ~d(v_{(x)}, v'_{(x)})$ & ~$\Leftrightarrow$~ & $\predicate = x_i \preceq k$ \\
$\mathlarger{\oplus}_{v' \models x_i \preceq k}  ~d(v_{(x_i)}, v'_{(x_i)})$ & ~$\Leftrightarrow$~ &    Def.~\ref{def:distance}\\

%$d(\val_{(x_i)}, k)$ & ~$\Leftrightarrow$~ &  Def.~\ref{def:distance} \\


\Bigg\{
\begin{tabular} {rl}
$\mathlarger{\oplus}_{v' \models x_i \preceq k \wedge v' \neq v} ~d(v_{(x_i)}, v'_{(x_i)}) \oplus ~d(v_{(x_i)}, v_{(x_i)}) $& ,if $v \models  x_i \preceq k $ \\
$\mathlarger{\oplus}_{v' \models x_i \preceq k}  ~d(v_{(x_i)}, v'_{(x_i)})$  &, otherwise 
%$\lVert x_i - k \rVert$&,otherwise \\
\end{tabular}
\Bigg\}  & ~$\Leftrightarrow$~ & Def.~\ref{def:distance}: (2) \\

\Bigg\{
\begin{tabular} {rl}
$\mathlarger{\oplus}_{v' \models x_i \preceq k \wedge v' \neq v} ~d(v_{(x_i)}, v'_{(x_i)}) \oplus ~\oone $& ,if $v \models  x_i \preceq k $ \\
$\mathlarger{\oplus}_{v' \models x_i \preceq k}  ~d(v_{(x_i)}, v'_{(x_i)})$  &, otherwise 
%$\lVert x_i - k \rVert$&,otherwise \\
\end{tabular}
\Bigg\}  & ~$\Leftrightarrow$~ & $\oone$ annihilates $\oplus$ \\


\Bigg\{
\begin{tabular} {rl}
$\oone$ & ,if $(x_i \preceq k)$ \\
$\mathlarger{\oplus}_{v' \models x_i \preceq k}  ~d(v_{(x_i)}, v'_{(x_i)})$  &, otherwise 
\end{tabular}
\Bigg\}  & ~$\Leftrightarrow$~ & Def.~\ref{def:distance}: (4)\\

\Bigg\{
\begin{tabular} {rl}
$\oone$& ,if $(x_i \preceq k)$ \\
$\lVert x_i - k \rVert$&,otherwise \\
\end{tabular}
\Bigg\} 

 

\end{tabular}

This is equivalent to the branch of Algorithm~\ref{alg:pred-val}, when $\predicate = x_i \preceq k$.% and $\oone = 0$.

\noindent \textit{Base Case 2}: Theorem~\ref{thm:valpred} holds for $\predicate = \neg (x \preceq k)$. 

Analog to Base Case 1. Exploits the norm symmetry $\lVert x_i - k \rVert = \lVert k - x_i \rVert$

\noindent \textit{Induction Hypothesis}: Theorem~\ref{thm:valpred} holds for arbitrary basic propositions $\predicate_1, \predicate_2$. 

\noindent \textit{Induction Step 1}: Theorem~\ref{thm:valpred} holds for an arbitrary  P-term  $\predicate = \predicate_1 \wedge \predicate_2$. 

The proof follows directly from Lemma~\ref{lemma1}.

\noindent \textit{Induction Step 2}: Theorem~\ref{thm:valpred} holds for an arbitrary minimal DNF $\predicate$. 

The proof follows directly from Lemma~\ref{lemma2}.


\end{proof} \qed


%-------------------------Theorem 2------------------------------------------------

\begin{nnlem}
\label{lemma3}
Let $\tau$ be a trace, $\waut$ a weighted symbolic automaton and 
$\pi_{1}$ and $\pi_{2}$ two paths
in $\waut$ induced by $\tau$ such that both paths terminate in the same state $q \in Q$ and $\pweight(\tau,\pi_{1}) < \pweight(\tau,\pi_{2})$. 
Then, for all continuations $\tau'$ of $\tau$ and all paths $\pi_{1} \cdot \pi$ and $\pi_{2} \cdot \pi$ induced by $\tau \cdot \tau'$, 
$\pweight(\tau \cdot \tau',\pi_{1} \cdot \pi) < \pweight(\tau \cdot \tau',\pi_{2} \cdot \pi)$.
\end{nnlem}

\begin{proof}
%The proof follows directly from the Myhill-Nerode theorem and the definition of the path value in a weighted automaton.
The proof follows directly from the definition of path and the definition of path value in weighted automaton $\waut$.
Each continuation path of either $\pi_{1}$ or $\pi_{2}$ must start from the state $q$. Since both $\pi_{1}$ and $\pi_{2}$ terminate at state q it means that all valuations from $\tau$ are consumed once state $q'$ is reached. For this reason, it is clear that only $\tau'$ affects transition weights in $\pi$. As a consequence, and by Definition~\ref{def:path_weight} the following holds: $\pweight(\tau \cdot \tau',\pi_{i} \cdot \pi) =  \pweight(\tau,\pi_{i}) \otimes \pweight(\tau', \pi)$.

By Definition~\ref{def:path_weight}, $\pweight(\tau,\pi)$ in $\waut$ is $\otimes$-product of non-negative transition weights on an ordered domain. Consequently: 
$\pweight(\tau,\pi_{1}) \otimes \pweight(\tau',\pi) < \pweight(\tau,\pi_{2}) \otimes \pweight(\tau',\pi)$.

\end{proof} \qed

\begin{customthm}{\ref{th:val}}
Given a weighted symbolic automaton $\waut$ defined over a semiring $S$ and a trace $\trace$, we have that $\textsf{val}(\tau, \waut) = \tvalue(\trace, \waut)$.
\end{customthm}

\begin{proof}
The algorithm $\textsf{val}(\tau, \waut)$ iteratively explores the paths in $\waut$ induced by $\trace$ and computes the path weights after reading the trace prefix. Although the number of paths grows with the number of iterations, by Lemma~\ref{lemma3} it 
is sufficient to keep in every iteration only the weights of reaching an arbitrary state $Q$, induced by the trace prefix. When the main loop of the algorithm terminates, the values associated to each state clearly correspond to the $\oplus$-sum values of reaching them with the signal $\trace$. The $\oplus$-sum of weights of all the paths ending in an accepting state hence corresponds to $\tvalue(\trace, \waut)$.

\end{proof} \qed


\begin{customthm}{\ref{th:qual}}
Given a trace $\trace$, a specification $\varphi$ and the Boolean semiring $S$, $\textsf{robustness}(\trace, \varphi) = 0$  iff  $\tau \models \varphi$ and 
$\textsf{robustness}(\trace, \varphi) = 1$ otherwise.
\end{customthm}

\begin{proof}
We prove this theorem by contradiction.

We start with a trace $\trace$ and $\waut_{\varphi}$.
It follows directly from Definitions~\ref{def:distance} and~\ref{def:path_weight} and Algorithms~\ref{alg:pred-val} and~\ref{alg:val} that when $\trace \models \varphi$ there exists a path which cost simply $\otimes$-multiplies $\oone$ weights. Then, the value of a trace in weighted symbolic automaton $\tvalue(\trace, \waut_{\varphi}) = \oone \mathlarger{\oplus}_{\path \in \paths(\trace)} \pweight(\trace, \path)$. Since $\oone$ is annihilator for $\oplus$, 
$\tvalue(\trace, \waut_{\varphi}) = \oone = 0$. 

Let's now assume there exists $\trace \not\models \varphi$ and for which $\tvalue(\trace, \waut_{\varphi}) = 0$. This implies that there is at least one accepthing path in $\waut_{\varphi}$ for which all the transitions taken on this path have weight $\oone = 0$. By construction of $\waut_{\varphi}$ and line 3 of Algorithm~\ref{alg:pred-val}, the cost of path induced by $\trace \not\models \varphi$ has at least one transition with predicate yielding $\lVert x - k \rVert $ weight for a given valuation from $\trace$. Thus, $\tvalue(\trace, \waut_{\varphi}) \neq 0$ and we reach a contradiction.

Symmetrically, we can prove the second part of the theorem by construction of $\waut_{\varphi}$ and the fact that operation $\otimes$ is closed on $\{ 0, 1 \}$.

\end{proof} \qed

\begin{nnlem}
\label{lemma4}
Given a trace $\trace$, Weighted Symbolic Automata $\waut_{\varphi}$ and $\waut_{\neg\varphi}$, constructed according to the procedure from Section~\ref{sec:translation} for specification $\varphi$ and its negation respectively, the following holds:
$$ \textsf{val}(\tau, \waut_{\varphi}) = 0  ~\vee~ \textsf{val}(\tau, \waut_{\neg\varphi}) = 0 $$
\end{nnlem}

\begin{proof}
Proof follows directly from $L(\varphi) \cap L(\neg\varphi) = \emptyset$
\end{proof} \qed




\begin{customthm}{\ref{th:fainekos_pappas}} 
Given a trace $\trace$, a specification $\varphi$ and semiring $S$, $\textsf{robustness}(\trace, \varphi)$ is precise:
$$
\textsf{robustness}(\trace, \varphi) > \oone  \Leftrightarrow \trace \models \varphi
$$
$$
\textsf{robustness}(\trace, \varphi) < \oone  \Leftrightarrow \trace \not\models \varphi
$$
\end{customthm}
\begin{proof}
We shall prove only the first equivalence, since the proof for the second equivalence is symmetric.

\begin{tabular}{crlrrl}
  & & & \\
     & &  $ \textsf{robustness}(\trace, \varphi) > \oone$  &   ~$\Leftrightarrow$~   &   Algorithm~\ref{alg:rob}, Lemma~\ref{lemma4}\\
     & $ \textsf{val}(\tau, \waut_{\varphi}) = \oone$   &   ~$\wedge$~                  $\textsf{val}(\tau, \waut_{\neg\varphi}) > \oone$    &   ~$\Leftrightarrow$~   &   Theorem~\ref{th:val}, Theorem~\ref{th:mon}\\
     & $ \trace \in L(\waut_{\varphi})                     $   &   ~$\wedge$~                  $\trace \not\in L(\waut_{\neg\varphi}) $		        	&   ~$\Leftrightarrow$~   &    \\
     & &  $ \trace \models \varphi$ &\\
\end{tabular}

\end{proof} \qed








==> proof2.tex <==

\section{Proof of Theorem~\ref{th:mon}}
\label{sec:proof_new}

In this appendix, we provide the proof that $d(\trace, \varphi) = \tvalue(\trace, \waut_{\varphi})$. 
We decompose the problem in the following way:


\begin{tabular}{crclc}
     & & & \\
     & $  d(\trace, \varphi)     $ 					          & $=$  & $\tvalue(\trace, \waut_{\varphi})$ 						& $\Leftrightarrow$ \\
\vspace{-5pt}\\
(1) & $  d(\trace, L(\varphi)) $ 					          & $=$  & $\tvalue(\trace, \bigcup\limits_{s \in L(\varphi)} \waut^{s})$  & $\Leftrightarrow$  \\
\vspace{-8pt}\\
(2) & $  \oplus_{s \in L(\varphi)}~d(\trace, s)$      	   & $=$   & $\oplus_{s \in L(\varphi)}~\tvalue(\trace,\waut^{s}) $ & $\Leftrightarrow$ \\
\vspace{-5pt}\\
(3) & $  	                                   d(\trace, s)$        	   & $=$   & $\tvalue(\trace,\waut^{s}) $  \\
&&&\\
\end{tabular}

where $s$  represents an arbitrary word from the language of formula $\varphi$.

In (1) we first decompose $\waut_{\varphi}$ into a (possibly infinite) union of symbolic weighted automata $\waut^{s}$, where each $\waut^{s}$ models 
a single word $s \in L(\varphi)$ and all the transitions preserve the weight functions from $\waut_{\varphi}$. Then, in (2) we show that calculating the $\oplus$-sum of distance between trace $\trace$ and each $s \in L(\varphi)$ 
is equivalent to calculating the $\oplus$-sum of values induced by $\trace$ in each of the $\waut^{s}$, where  $s \in L(\varphi)$. Finally, in (3) we show that for an arbitrary $s$, the 
distance $d(\trace,s)$ is equivalent to the value $\tvalue(\trace,\waut^{s})$. We proceed in the bottom up fashion, by first proving relation (3).

\begin{definition}
\label{def:SWA}
Given a word $s$, we define a {\em single word acceptor} for $s$, $\aut^s$, as the minimal automaton such that $L(\aut^s) = \{s\}$ holds. 
%We denote by $\waut^{s}$ the {\em single word weighted symbolic automaton} (SWWSA) which is constructed  by augmenting transitions in $\aut^{s}$ 
%with distance metrics as weight functions ( Definition~\ref{def:distance}).
\end{definition}
\begin{definition}
\label{def:SWWSA}
Given an single word acceptor $\aut^s$, we define the {\em single word  symbolic weighted automaton} (SWSWA $\waut^{s}$ by augmenting transitions in $\aut^{s}$ 
with distance metrics as weight functions (Definition~\ref{def:distance}), such that the word $s$ induces only one zero weight accepting path in $\waut^{s}$.
\end{definition}

We note that for every $s$ of size $n$, both $\aut^{s}$ and $\waut^{s}$ consist of a sequence of locations $q_{0},\ldots, q_{n}$, where $q_{0}$ is 
the only initial location, $q_{n}$ is the only final location, and for all $0 < i \leq n$, the incoming transitions to $q_{i}$ have a source either in $q_{i-1}$ or in $q_{i}$. 
We define by $P(s)$ the set of all prefixes of a signal $s$, where $s[0,i)$ denotes the prefix of $s$ of size $i$, where $0 \leq i \leq |s|$. 

% --------------- to be considered ? 
%In F I G%Figure~\ref{fig:wk}, 
%we illustrate the array of weighted edit automata $\waut^{s[0,i)}$ for the prefixes of the signal $s$ of size $4$. 
%I N P U T   W K
%\input{wk}

\begin{nnlem} 
\label{eee}
Let $s$ and $s'$ be two arbitrary words of size $n$ and let  $\waut^{s'[0,i)}$ designate SWSWA for word prefix $s'[0,i)$. Then, for all $0 \leq i \leq n$, we have that 
$d(s[0,i),s'[0,i)) = \tvalue(s[0,i), \waut^{s'[0,i)})$. 
\end{nnlem}

\begin{proof}

The proof follows directly from Definitions~\ref{def:distance},~\ref{def:wsa},~\ref{def:path_weight}.

\end{proof} \qed


\begin{corollary}
\label{fff}
$d(\trace,s) = \tvalue(\trace, \waut^{s})$
\end{corollary}


%We prove this lemma by induction.
%
%\noindent \emph{Base case:} We first prove that (1) $d_W(\epsilon, s'[0,j)) = v(\epsilon, \waut^{s'[0,j)})$ for all $0 \leq j \leq n$ and 
%(2) $d_W(s[0,i), \epsilon) = v(s[0,i), \waut^{\epsilon})$ for all $0 \leq i \leq m$. 
%In the case (1), by the definition of the weighted edit distance  $d_W(\epsilon, s'[0,j)) = jc_{i}$.  
%The cheapest path from the initial to the finite location in $\waut^{s'[0,j)}$ induced by an empty word is by taking $j$ consecutive $\epsilon$ (insertion) 
%transition, each inducing a cost of $c_i$. In the case (2), by the definition of the weighted edit distance $d_W(s[0,i), \epsilon) = ic_{d}$. 
%The cheapest path from the initial to the accepting state in $\waut^{\epsilon}$ induced by $s[0,i)$ is to consume the $i$ letters by consecutive self-loop (deletion) 
%transition, each inducing a cost of $c_d$.
%
%\noindent \emph{Inductive step:}  By inductive hypothesis, we assume that 
%$d(s[0,i-1),s'[0,j-1)) = v(s[0,i-1), \waut^{s'[0,j-1)})$, $d(s[0,i-1),s'[0,j)) = v(s[0,i-1), \waut^{s'[0,j)})$ and 
%$d(s[0,i),s'[0,j-1)) = v(s[0,i), \waut^{s'[0,j-1)})$. We now prove that $d(s[0,i),s'[0,j)) = v(s[0,i), \waut^{s'[0,j)})$. 
%By definition of the weighted edit distance, we have that
%$$
%\begin{tabular}{lll}
%
%$d_W(s[0,i),s'[0,j))$    &     $=$    &
% $ min \left\{
%  \begin{tabular}{ll}
% $d_{W}(s[0,i-1), s'[0,j-1))$ & $+ c_{s}(s(i), s'(j))$\\
% $d_{W}(s[0,i),s'[0,j-1))$    & $+ c_{i}  $\\
% $d_{W}(s[0,i-1),s'[0,j))$    & $+ c_{d} $\\
% \end{tabular}
%\right.$
%\end{tabular}
%$$
%
%
%
%
%
%
%
%We now prove that
%
%$$
%\begin{tabular}{lll}
%
%$v(s[0,i),\waut^{s'[0,j)})$    &     $=$    &
% $ min \left\{
%  \begin{tabular}{ll}
% $v(s[0,i-1),\waut^{s'[0,j-1)})$ & $+ c_{s}(s(i), s'(j))$\\
% $v(s[0,i),\waut^{s'[0,j-1)})$    & $+ c_{i}  $\\
% $v(s[0,i-1),\waut^{s'[0,j)})$    & $+ c_{d} $\\
% \end{tabular}
%\right.$
%\end{tabular}
%$$
%
%
%
%
%We first observe that $\waut^{s'[0,j)}$ has only one final location $q_j$. By the definition of the weighted symbolic automata,
%path values are non-negative and additive, and by the definition of $\waut^{s'[0,j)}$, any location $q_{j'}$, where $0 < j' \leq j$ 
%can be reached in one step only from $q_{j'}$ or $q_{j' -1}$. It follows that it is sufficient to consider $s[0,i)$ and $s[0,i-1)$ and 
%$q_{j}$ and $q_{j-1}$ in order to prove $d(s[0,i),s'[0,j)) = v(s[0,i), \waut^{s'[0,j)})$.
%Let $\pi = \pi' \cdot \delta \cdot q_j$ be the path with minimum value induced by $s[0,i)$ in $\waut^{s'[0,j)}$. 
%By the the definition of $\waut^{s'[0,j)}$, $q_j$ has $3$ incoming transitions: 
%(1) a substitution transition from $q_{j-1}$ to $q_{j}$; 
%(2) an $\epsilon$ (insertion) transition from $q_{j-1}$ to $q_j$; and 
%(3) a self-loop (deletion) transition in from $q_j$ to $q_j$.
%
%By the definition of the value in a weighted symbolic automaton, the value of $\pi$ corresponds to the value 
%
%of $\pi'$ to which the cost of the last transition $\delta$ is added, which is the minimum of the above three cases.  
%In the case (1), $\pi'$ reaches $q_{j-1}$ with $s[0,i-1)$ consumed. The value accumulated by $\pi'$ corresponds to the 
%value of $\pi'$ induced by $s[0,i-1)$ in $\waut^{s'[0,j-1)}$, i.e. $v(s[0,i-1),\waut^{s'[0,j-1)})$. The added 
%cost of the last transition corresponds to $c_{s}(s(i), s'(j))$. In the case (2), $\pi'$ reaches $q_{j-1}$ with $s[0,i)$ consumed. 
%The value accumulated by $\pi'$ corresponds to the 
%value of $\pi'$ induced by $s[0,i)$ in $\waut^{s'[0,j-1)}$, i.e. $v(s[0,i),\waut^{s'[0,j-1)})$. 
%The added cost of the last transition corresponds to the cost $c_i$ of an insertion. 
%In the case (3), $\pi'$ reaches $q_{j}$ with $s[0,i-1)$ consumed. 
%The value accumulated by $\pi'$ corresponds to the 
%value of $\pi'$ induced by $s[0,i-1)$ in $\waut^{s'[0,j)}$, i.e. $v(s[0,i-1),\waut^{s'[0,j)})$. 
%The added cost of the last transition corresponds to the cost $c_d$ of a deletion.


%\end{proof} \qed


\noindent Corollary~\ref{fff} is a special case of Lemma~\ref{eee}, where $i=n$. We can now generalize Corollary~\ref{fff} with the following 
lemma, in order to take into account all the (possibly infinite number of) words that are in the language of STL formula $\varphi$.

\begin{nnlem} 
\label{ggg}
$ \oplus_{s \in L(\varphi)} d(\trace,s) = \oplus_{s \in L(\varphi)} \tvalue(\trace, \waut^{s})$
%$\min_{s' \in L(\varphi)} d_W(s,s') = \min_{s' \in L(\varphi)}v(s, \waut^{s'})$.
\end{nnlem}

\begin{proof}
Follows directly from Corollary~\ref{fff} and Definition~\ref{def:semiring}.
\end{proof} \qed

\begin{corollary}
\label{kkk}
$d(\trace, L(\varphi)) = \tvalue(\trace, \bigcup\limits_{s \in L(\varphi)} \waut^{s})$


\end{corollary}

\noindent The above corollary follows from Definition~\ref{def:distance}, and %the fact that $\oplus$ distributes over the union?
 language equivalence $L(\varphi) = \bigcup\limits_{s \in L(\varphi)} L(\waut^{s})$.

We finally need to show that the decomposition of $\waut_{\varphi}$ into $\bigcup_{s \in L(\varphi)}\waut^{s}$ preserves the paths and the corresponding 
weights induced by $s$.

\begin{nnlem} 
\label{hhhhhh}
Consider an arbitrary trace $\trace$ and an STL formula $\varphi$. For every path $\pi$ in $\waut_{\varphi}$ induced by $\trace$, there exists $\pi'$ in 
$\bigcup_{s \in L(\varphi)} \waut^{s}$ induced by $\trace$, and for every path  $\pi'$ in 
$\bigcup_{s \in L(\varphi)} \waut^{s}$ induced by $\trace$, there exists a path $\pi$ in $\waut_{\varphi}$ induced by $\trace$, such that
$\pweight_{\pi}(\trace,\waut_{\varphi}) = \pweight_{\pi'}(\trace, \bigcup_{s \in L(\varphi)} \waut^{s})$.
\end{nnlem}

\begin{proof}
We create a SWSWA $\waut^{s}$ for every word $s \in L(\varphi)$. By construction, it follows that $\bigcup_{s \in L(\varphi)} \waut^{s}$ contains exactly the same paths 
as $\waut_{\varphi}$. By construction, path weights $\pweight$ are also preserved.
\end{proof} \qed

\begin{nnlem} 
\label{hhh}
$\tvalue(\trace,\waut_{\varphi}) = \tvalue(\trace, \bigcup_{s \in L(\varphi)}\waut^{s})$.
\end{nnlem}

\begin{proof}
Follows directly from the preservation of all paths and their values proved in Lemma~\ref{hhhhhh} and the Definition~\ref{def:path_weight}.
\end{proof} \qed

The combination of Lemma~\ref{hhh}, Corollary~\ref{kkk}, Lemma~\ref{ggg} and Corollary~\ref{fff} constitutes the proof of Theorem~\ref{th:mon}.


==> properties.tex <==
\section{Monitor Properties}
\label{sec:properties}

\begin{table}[htb]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Semantics & $d(x,x')$ & $S_{\circ}$ & $S_{\Box}$ \\
\hline
\hline
Qualitative & $x \equiv x'$ & Boolean & Boolean \\
$\infty$-norm & $\lVert x - x' \rVert$ & Min Max & Min Max \\
Hamming & $\lVert x - x' \rVert$ & Tropical & Tropical \\
\hline
\end{tabular}
\caption{Monitor instantiations.}
\label{sec:instant}
\end{table}
